Asymmetric predictability in causal discovery: an information theoretic approach

Causal investigations in observational studies pose a great challenge in research where randomized trials or intervention-based studies are not feasible. We develop an information geometric causal discovery and inference framework of "predictive asymmetry". For $(X, Y)$, predictive asymmetry enables assessment of whether $X$ is more likely to cause $Y$ or vice-versa. The asymmetry between cause and effect becomes particularly simple if $X$ and $Y$ are deterministically related. We propose a new metric called the Directed Mutual Information ($DMI$) and establish its key statistical properties. $DMI$ is not only able to detect complex non-linear association patterns in bivariate data, but also is able to detect and infer causal relations. Our proposed methodology relies on scalable non-parametric density estimation using Fourier transform. The resulting estimation method is manyfold faster than the classical bandwidth-based density estimation. We investigate key asymptotic properties of the $DMI$ methodology and a data-splitting technique is utilized to facilitate causal inference using the $DMI$. Through simulation studies and an application, we illustrate the performance of $DMI$.

==> ENAR_Mengtong__Copy_/Method_comparison_tab.tex <==
\begin{table}[]
\begin{tabular}{lccc}
\hline
       & \begin{tabular}[c]{@{}c@{}}Propensity Score \\ (PS)\end{tabular}                                                                    & \begin{tabular}[c]{@{}c@{}}Causal Effect \\ (ATE)\end{tabular}                                                                                                     & \begin{tabular}[c]{@{}c@{}}Information Matrices \\ (INF)\end{tabular}                                                                                                                              \\ \hline
3R-GLO & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Round 1: PS\\  $\hat{\gamma}^{\myinc \star}$\\ $\newline$\\ $\newline$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Round 2: ATE\\  $\tilde{\beta}^{\myinc \star}(\hat{\gamma}^{\myinc \star})$\\ $\newline$\\ $\newline$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Round 3: INF\\ $\HNKtilde=\sum_{j=1}^k{H}_{n_j}(\incgammaall, \incbetaall) $\\  $ \VNKtilde=\sum_{j=1}^k{V}_{n_j}(\incgammaall, \incbetaall)$\\ $\newline$\end{tabular} \\ \hline
2R-GLO & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Round 1: PS\\ $\hat{\gamma}^{\myinc \star}$\\ $\newline$\\ $\newline$\end{tabular}}  & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Round 2: ATE + INF\\ $\tilde{\beta}^{\myinc k}(\hat{\gamma}^{\myinc \star})$\\ $\HNKbreve=\sum_{j=1}^k{H}_{j}(\incgammaall, \incbetak) $,  and $ \VNKbreve=\sum_{j=1}^k{V}_{j}(\incgammaall, \incbetak)$\\ $\newline$\end{tabular}}                                                                                       \\ \hline
1R-GLO & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Round 1: PS + ATE + INF\\ $\hat{\gamma}^{\myinc k}$, $\hat{\beta}^{\myinc k}(\hat{\gamma}^{\myinc k})$,\\ $\HNK=\sum_{j=1}^k{H}_{j}(\hatincgammak, \hat{\beta}^{\myinc k}) \mbox{ , and }$ $ \VNK=\sum_{j=1}^k{V}_{j}(\hatincgammak, \hat{\beta}^{\myinc k})$\end{tabular}}                                                                                                                                                                                     \\ \hline
\end{tabular}
\caption{A comparison of estimates obtained from 3R-GLO, 2R-GLO, and 1R-GLO. We use $\star$ to denote the global estimate for the parameter which is obtained by a full round of sequential updating method. 3R-GLO and 2R-GLO will output the same point estimates for PS and ATE. The information matrices thus the asymptotic covariances obtained from these three algorithms are slightly different. }
\label{tab:compare}
\end{table}

==> ENAR_Mengtong__Copy_/algorithm_table.tex <==
\begin{algorithm}[H]
		\caption{Two-rounds (2R-GLO) implementation of collaborative inference algorithm}     	
		\label{tab:algo_tab}
		\begin{algorithmic}[1]\setstretch{1}
     			\State \textbf{Round 1:} 
     			\For {$k \in \{1, 2, 3 \hdots K\} $}
				\Input \Desc{$A_k,X_k,\hat{\gamma}^{\myinc k-1},\mbox{ and }\widehat{H}^{\text{ps}}_{N_{k-1}}$}
				\EndInput
		    	\Output  	
			        \Desc{$\hat{\gamma}^{\myinc k}$}{~~the incremental PS model coefficients }
		        	\Desc{$\widehat{H}^{\text{ps}}_{N_k}$}{~~the incremental sensitivity matrix for the PS model}  
		    	\EndOutput 
			    \State \textbf{Run until Convergence}
			$\hat{\gamma}^{\myinc k(r)}=\hat{\gamma}^{\myinc k(r-1)}+\left\{ \widehat{H}^{\text{ps}}_{N_{k-1}}+{H}^{\text{ps}}_{n_{k}}(\hat{\gamma}^{\myinc k(r-1)})\right\}^{-1} \hat{\Phi}^{\myinc k(r-1)} ,$ \\ \qquad \qquad \qquad where $ \hat{\Phi}^{\myinc k(r-1)} = \left\{ \widehat{H}^{\text{ps}}_{N_{k-1}}(\hat{\gamma}^{\myinc k-1}-\hat{\gamma}^{\myinc k(r-1)})+U_{n_k}^{\text{ps}}(\hat{\gamma}^{\myinc k(r-1)})\right\}$
			    \State \textbf{Update} 
			$\widehat{H}^{\text{ps}}_{N_k}=\widehat{H}^{\text{ps}}_{N_{k-1}}+{H}^{\text{ps}}_{n_k}(\hat{\gamma}^{\myinc k})$
		    	\EndFor
		    \Output  	
			        \Desc{$\hat{\gamma}^{\myinc \star}$}{~~the global estimate of the PS model parameter}
			\EndOutput 
		    	\\
			\State \textbf{Round 2:} 
            \For {$k \in \{1, 2, 3 \hdots K\} $}
            	\Input \Desc{$A_k,X_k,Y_k,\hat{\gamma}^{\myinc \star}, \tilde{\omega}_{o}^{\myinc k-1},\tilde{\omega}_{1}^{\myinc k-1},\tilde{v}_{o}^{\myinc k-1},\tilde{v}_{1}^{\myinc k-1},\breve{\mathbb{H}}_{N_{k-1}} , \mbox{ and } \breve{\mathbb{V}}_{N_{k-1}} $}
				\EndInput
		    	\Output  	
		    	 \Desc{$\tilde{\omega}_{o}^{\myinc k},\tilde{\omega}_{1}^{\myinc k},\tilde{v}_{o}^{\myinc k},\tilde{v}_{1}^{\myinc k}$,  $\breve{\mathbb{H}}_{N_{k-1}} $, and $\breve{\mathbb{V}}_{N_{k-1}}$ }
			     %   \Desc{$\tilde{H}^{\myinc k-1}$}{~~~~~the incremental sensitivity matrix for overall estimating equations }
		      %  	\Desc{$\tilde{V}^{\myinc k-1}$}{~~~~the incremental variability matrix for overall estimating equations}
		    	\EndOutput 
		    	\Update \setstretch{1.4}
		    	\State$\tilde{\omega}_0^{\myinc k} = \tilde{\omega}_0^{\myinc k-1} + \sum_{i=1}^{n_k} \frac{1-A_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})} , \quad \tilde{\omega}_1^{\myinc k} = \tilde{\omega}_1^{\myinc k-1} + \sum_{i=1}^{n_k} \frac{A_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})} $
		    		\State$\tilde{v}_0^{\myinc k} = \tilde{v}_0^{\myinc k-1} + \sum_{i=1}^{n_k} \frac{(1-A_{ki})Y_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})} , \quad \tilde{v}_1^{\myinc k} = \tilde{v}_1^{\myinc k-1} + \sum_{i=1}^{n_k} \frac{A_{ki}Y_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})} $
		    		\State $\tilde{\mu}_{0}^{\myinc k}=  \tilde{v}_0^{\myinc k}/\tilde{\omega}_0^{\myinc k}, \quad \quad \tilde{\mu}_{1}^{\myinc k}=  \tilde{v}_1^{\myinc k}/\tilde{\omega}_1^{\myinc k}$
% 		    	\State $\tilde{\mu}_{0}^{\myinc k}=\tilde{\mu}_{0}^{\myinc k-1}+ (\sum_{i=1}^{n_k} \frac{(1-A_{ki})}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})})^{-1}\sum_{i=1}^{n_k} \frac{(1-A_{ki}) Y_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})} $
% \State
%     $\tilde{\mu}_{1}^{\myinc k}=\tilde{\mu}_{1}^{\myinc k-1}+ (\sum_{i=1}^{n_k} \frac{A_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})})^{-1}\sum_{i=1}^{n_k} \frac{A_{ki} Y_{ki}}{\hat{e}_{ki}(X_{ki}; \hat{\gamma}^{\myinc \star})} $
\State
    $\tilde{\beta}_{A}^{\myinc k}=log\{\tilde{\mu}_{1}^{\myinc k}/(1-\tilde{\mu}_{1}^{\myinc k})\}-log\{\tilde{\mu}_{0}^{\myinc k}/(1-\tilde{\mu}_{0}^{\myinc k})\}$
\State    $\tilde{\beta}_{0}^{\myinc k}=log\{\tilde{\mu}_{0}^{\myinc k}/(1-\tilde{\mu}_{0}^{\myinc k})\}$
\State$\tilde{\theta}^{\myinc k} = (\hat{\gamma}^{\myinc \star},\tilde{\beta}_{A}^{\myinc k},\tilde{\beta}_{0}^{\myinc k})^{\top} $
\State  $\HNKbreve=\breve{\mathbb{H}}_{N_{k-1}}+{H}_{n_k}(\tilde{\theta}^{\myinc k})$ 
\State  $\VNKbreve=\breve{\mathbb{V}}_{N_{k-1}}+{V}_{n_k}(\tilde{\theta}^{\myinc k})$
\EndUpdate
            \EndFor
           \State{\textbf{Final Output}}  $\tilde{\beta}_{A}^{\myinc \star}$ and $    \breve{J}_{N_k}(\tilde{\theta}^{\myinc \star})=
N_k(\HNKbreve^{\top} \VNKbreve \HNKbreve)$
		\end{algorithmic}
	\end{algorithm}

	



==> ENAR_Mengtong__Copy_/data_example_fig.tex <==

\begin{figure}[H]
    \centering

\includegraphics[width=\columnwidth]{data_example_graph.eps} 
% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

% %Shape: Rectangle [id:dp37753686177454515] 
% \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (55.5,124.54) -- (132.86,124.54) -- (132.86,155.01) -- (55.5,155.01) -- cycle ;
% %U Turn Arrow [id:dp3102808793868894] 
% \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (87.83,125.34) -- (87.83,117.13) .. controls (87.83,115.11) and (89.47,113.47) .. (91.49,113.47) -- (236.92,113.47) .. controls (238.94,113.47) and (240.58,115.11) .. (240.58,117.13) -- (240.58,119.58) -- (241.77,119.58) -- (238.8,122.97) -- (235.83,119.58) -- (237.02,119.58) -- (237.02,117.13) .. controls (237.02,117.08) and (236.97,117.03) .. (236.92,117.03) -- (91.49,117.03) .. controls (91.44,117.03) and (91.39,117.08) .. (91.39,117.13) -- (91.39,125.34) -- cycle ;
% %U Turn Arrow [id:dp43350675757855117] 
% \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (245.55,123.29) -- (245.55,115.82) .. controls (245.55,113.98) and (247.05,112.49) .. (248.89,112.49) -- (395.08,112.49) .. controls (396.92,112.49) and (398.41,113.98) .. (398.41,115.82) -- (398.41,118.04) -- (399.49,118.04) -- (396.79,121.13) -- (394.09,118.04) -- (395.17,118.04) -- (395.17,115.82) .. controls (395.17,115.77) and (395.13,115.73) .. (395.08,115.73) -- (248.89,115.73) .. controls (248.84,115.73) and (248.8,115.77) .. (248.8,115.82) -- (248.8,123.29) -- cycle ;
% %U Turn Arrow [id:dp6483835598496202] 
% \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (408.98,123.67) -- (408.98,115.94) .. controls (408.98,114.03) and (410.52,112.49) .. (412.43,112.49) -- (536.14,112.49) .. controls (538.05,112.49) and (539.59,114.03) .. (539.59,115.94) -- (539.59,118.24) -- (540.71,118.24) -- (537.91,121.44) -- (535.12,118.24) -- (536.24,118.24) -- (536.24,115.94) .. controls (536.24,115.89) and (536.19,115.84) .. (536.14,115.84) -- (412.43,115.84) .. controls (412.38,115.84) and (412.33,115.89) .. (412.33,115.94) -- (412.33,123.67) -- cycle ;
% %U Turn Arrow [id:dp23820460197159665] 
% \draw   (534.19,173.73) -- (534.19,182.62) .. controls (534.19,184.81) and (532.41,186.59) .. (530.22,186.59) -- (407.71,186.59) .. controls (405.52,186.59) and (403.74,184.81) .. (403.74,182.62) -- (403.74,179.97) -- (402.46,179.97) -- (405.67,176.3) -- (408.88,179.97) -- (407.6,179.97) -- (407.6,182.62) .. controls (407.6,182.68) and (407.65,182.73) .. (407.71,182.73) -- (530.22,182.73) .. controls (530.28,182.73) and (530.33,182.68) .. (530.33,182.62) -- (530.33,173.73) -- cycle ;
% %U Turn Arrow [id:dp5629342247285605] 
% \draw   (394.13,173.41) -- (394.13,182.52) .. controls (394.13,184.77) and (392.31,186.59) .. (390.06,186.59) -- (245.57,186.59) .. controls (243.33,186.59) and (241.51,184.77) .. (241.51,182.52) -- (241.51,179.81) -- (240.19,179.81) -- (243.48,176.04) -- (246.78,179.81) -- (245.46,179.81) -- (245.46,182.52) .. controls (245.46,182.58) and (245.51,182.63) .. (245.57,182.63) -- (390.06,182.63) .. controls (390.12,182.63) and (390.17,182.58) .. (390.17,182.52) -- (390.17,173.41) -- cycle ;
% %U Turn Arrow [id:dp8129735574945136] 
% \draw   (240.19,175.4) -- (240.19,183.13) .. controls (240.19,185.04) and (238.64,186.59) .. (236.74,186.59) -- (90.82,186.59) .. controls (88.91,186.59) and (87.37,185.04) .. (87.37,183.13) -- (87.37,180.83) -- (86.25,180.83) -- (89.04,177.64) -- (91.84,180.83) -- (90.72,180.83) -- (90.72,183.13) .. controls (90.72,183.19) and (90.76,183.23) .. (90.82,183.23) -- (236.74,183.23) .. controls (236.79,183.23) and (236.83,183.19) .. (236.83,183.13) -- (236.83,175.4) -- cycle ;
% %Shape: Rectangle [id:dp3797238027742196] 
% \draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (258.25,84) -- (411.59,84) -- (411.59,105.98) -- (258.25,105.98) -- cycle ;
% %Shape: Rectangle [id:dp18637295002718468] 
% \draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ] (262.43,191.5) -- (417.32,191.5) -- (417.32,214) -- (262.43,214) -- cycle ;
% %Shape: Rectangle [id:dp5061030159930031] 
% \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (204.08,125.49) -- (281.45,125.49) -- (281.45,155.95) -- (204.08,155.95) -- cycle ;
% %Shape: Rectangle [id:dp7189804419005674] 
% \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (351.44,125.49) -- (428.8,125.49) -- (428.8,155.95) -- (351.44,155.95) -- cycle ;
% %Shape: Rectangle [id:dp7219311601084708] 
% \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (499.64,125.49) -- (577,125.49) -- (577,155.95) -- (499.64,155.95) -- cycle ;

% % Text Node
% \draw (70.88,131.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {Berlin};
% % Text Node
% \draw (310,89.86) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Round 1};
% % Text Node
% \draw (312.13,195.42) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] { Round 2};
% % Text Node
% \draw (212.03,132.36) node [anchor=north west][inner sep=0.75pt]   [align=left] {Barcelona};
% % Text Node
% \draw (363.76,132.36) node [anchor=north west][inner sep=0.75pt]   [align=left] {Vienna};
% % Text Node
% \draw (521.77,132.36) node [anchor=north west][inner sep=0.75pt]   [align=left] {Graz};
% % Text Node
% \draw (74.85,156.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {n=86};
% % Text Node
% \draw (223.31,156.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {n=63};
% % Text Node
% \draw (377.44,155.37) node [anchor=north west][inner sep=0.75pt]   [align=left] {n=33};
% % Text Node
% \draw (517.39,156.31) node [anchor=north west][inner sep=0.75pt]   [align=left] {n=25};


% \end{tikzpicture}
% \caption{A diagram showing the the incremental update algorithm used in ITP-NODAT. The position of hospitals in the incremental sequence is determined by the local sample size. The starting site is Charité Universitätsmedizin Berlin, Germany where 89 participants are recruited followed by  Hospital del Mar Barcelona, Spain and Medical
% Universities of Vienna and Graz, Austria.Dashed arrows indicate the steps that incrementally update propensity score model estimates and solid arrows indicate the steps that incrementally update the causal log odds ratio of the treatment and its corresponding variance.  }
\caption{ITP-NODAT data example summary statistics: a) the distribution of positive PTDM cases at four hospitals by control and treatment group. b) The decent overlap of incremental propensity score estimates between treated and control groups indicating the propensity score weighted treatment and control groups are likely to be comparable, justifying the validity of our study } 
    \label{data:descp}

\end{figure}

==> ENAR_Mengtong__Copy_/intro_diagram.tex <==

\begin{figure}[t]
 \hspace*{-3.5cm}\includegraphics[width=1.4\columnwidth,trim={0 10cm 0 6cm},clip]{Graphs_ENAR.eps}
    
    \caption{A diagram showing '1R-GLO', '2R-GLO`, and '3R-GLO' algorithms of the collaborative inference method. The types of the arrows indicate the major updates involved in each update round: solid arrows always involve PS updates;  dashed arrows indicate average treatment effect estimates updating; dotted arrows represent incremental inference;. a) '1R-GLO' is a one around updating algorithm with the least amount of communication cost and achieves PS, ATE and inference updates simultaneously. b) '2R-GLO' involves two-round updates where the first round indicated by solid arrows produces global PS estimates, and the second round indicated by dot-dashed arrows updates the global causal effects and its variance. c) '3R-GLO' involves three-round updates, where the variance estimation uses result that is based on global propensity score estimates (solid arrows) and global causal estimates (dashed arrows).}
    \label{fig:my_label}
\end{figure}


% \begin{figure}[H]
%     \centering


% \label{fig:fig1}


% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% % \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% % %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

% % %Shape: Rectangle [id:dp19467274572367943] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (77.5,95.93) -- (103.24,95.93) -- (103.24,123.42) -- (77.5,123.42) -- cycle ;
% % %U Turn Arrow [id:dp06067635520208192] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (88.26,95.8) -- (88.26,88.39) .. controls (88.26,86.57) and (89.74,85.09) .. (91.56,85.09) -- (135.11,85.09) .. controls (136.94,85.09) and (138.42,86.57) .. (138.42,88.39) -- (138.42,90.6) -- (139.49,90.6) -- (136.81,93.66) -- (134.13,90.6) -- (135.2,90.6) -- (135.2,88.39) .. controls (135.2,88.34) and (135.16,88.3) .. (135.11,88.3) -- (91.56,88.3) .. controls (91.51,88.3) and (91.47,88.34) .. (91.47,88.39) -- (91.47,95.8) -- cycle ;
% % %U Turn Arrow [id:dp4282143269440657] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (140.75,93.95) -- (140.75,87.21) .. controls (140.75,85.55) and (142.09,84.2) .. (143.75,84.2) -- (187.99,84.2) .. controls (189.65,84.2) and (191,85.55) .. (191,87.21) -- (191,89.22) -- (191.98,89.22) -- (189.54,92) -- (187.1,89.22) -- (188.08,89.22) -- (188.08,87.21) .. controls (188.08,87.16) and (188.04,87.13) .. (187.99,87.13) -- (143.75,87.13) .. controls (143.71,87.13) and (143.67,87.16) .. (143.67,87.21) -- (143.67,93.95) -- cycle ;
% % %U Turn Arrow [id:dp5002878625362621] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (195.13,94.29) -- (195.13,87.32) .. controls (195.13,85.6) and (196.53,84.2) .. (198.25,84.2) -- (234.85,84.2) .. controls (236.57,84.2) and (237.96,85.6) .. (237.96,87.32) -- (237.96,89.39) -- (238.97,89.39) -- (236.45,92.28) -- (233.92,89.39) -- (234.93,89.39) -- (234.93,87.32) .. controls (234.93,87.27) and (234.89,87.23) .. (234.85,87.23) -- (198.25,87.23) .. controls (198.2,87.23) and (198.16,87.27) .. (198.16,87.32) -- (198.16,94.29) -- cycle ;
% % %U Turn Arrow [id:dp6886265488106063] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (276.88,94.29) -- (276.88,87.32) .. controls (276.88,85.6) and (278.27,84.2) .. (279.99,84.2) -- (304.41,84.2) .. controls (306.13,84.2) and (307.53,85.6) .. (307.53,87.32) -- (307.53,89.39) -- (308.54,89.39) -- (306.01,92.28) -- (303.49,89.39) -- (304.5,89.39) -- (304.5,87.32) .. controls (304.5,87.27) and (304.46,87.23) .. (304.41,87.23) -- (279.99,87.23) .. controls (279.94,87.23) and (279.9,87.27) .. (279.9,87.32) -- (279.9,94.29) -- cycle ;
% % %U Turn Arrow [id:dp11254614871038382] 
% % \draw   (307.7,125.16) -- (307.7,133.81) .. controls (307.7,135.94) and (305.97,137.67) .. (303.84,137.67) -- (278.44,137.67) .. controls (276.31,137.67) and (274.58,135.94) .. (274.58,133.81) -- (274.58,131.24) -- (273.33,131.24) -- (276.46,127.66) -- (279.59,131.24) -- (278.34,131.24) -- (278.34,133.81) .. controls (278.34,133.87) and (278.38,133.92) .. (278.44,133.92) -- (303.84,133.92) .. controls (303.9,133.92) and (303.95,133.87) .. (303.95,133.81) -- (303.95,125.16) -- cycle ;
% % %U Turn Arrow [id:dp7474064894698926] 
% % \draw   (235.23,126.67) -- (235.23,134.69) .. controls (235.23,136.66) and (233.62,138.27) .. (231.65,138.27) -- (196.13,138.27) .. controls (194.15,138.27) and (192.55,136.66) .. (192.55,134.69) -- (192.55,132.3) -- (191.39,132.3) -- (194.29,128.99) -- (197.19,132.3) -- (196.03,132.3) -- (196.03,134.69) .. controls (196.03,134.74) and (196.07,134.79) .. (196.13,134.79) -- (231.65,134.79) .. controls (231.7,134.79) and (231.75,134.74) .. (231.75,134.69) -- (231.75,126.67) -- cycle ;
% % %U Turn Arrow [id:dp6214108251957413] 
% % \draw   (188.62,126.38) -- (188.62,134.6) .. controls (188.62,136.62) and (186.97,138.27) .. (184.95,138.27) -- (142.25,138.27) .. controls (140.22,138.27) and (138.58,136.62) .. (138.58,134.6) -- (138.58,132.15) -- (137.39,132.15) -- (140.36,128.75) -- (143.33,132.15) -- (142.14,132.15) -- (142.14,134.6) .. controls (142.14,134.65) and (142.19,134.7) .. (142.25,134.7) -- (184.95,134.7) .. controls (185,134.7) and (185.05,134.65) .. (185.05,134.6) -- (185.05,126.38) -- cycle ;
% % %U Turn Arrow [id:dp6676289314694182] 
% % \draw   (137.39,128.17) -- (137.39,135.15) .. controls (137.39,136.87) and (135.99,138.27) .. (134.27,138.27) -- (90.28,138.27) .. controls (88.56,138.27) and (87.17,136.87) .. (87.17,135.15) -- (87.17,133.08) -- (86.16,133.08) -- (88.68,130.19) -- (91.2,133.08) -- (90.2,133.08) -- (90.2,135.15) .. controls (90.2,135.2) and (90.23,135.24) .. (90.28,135.24) -- (134.27,135.24) .. controls (134.32,135.24) and (134.36,135.2) .. (134.36,135.15) -- (134.36,128.17) -- cycle ;
% % %Down Arrow [id:dp36282265139114855] 
% % \draw   (388.77,90.72) -- (390.3,89.39) -- (378.25,75.6) -- (381.3,72.94) -- (393.35,86.73) -- (394.88,85.39) -- (396.43,93.33) -- cycle ;
% % %Shape: Rectangle [id:dp7210534640785944] 
% % \draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (144.97,58.5) -- (196,58.5) -- (196,78.33) -- (144.97,78.33) -- cycle ;
% % %Shape: Rectangle [id:dp6537684210080925] 
% % \draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ] (144.79,142.7) -- (196.33,142.7) -- (196.33,163) -- (144.79,163) -- cycle ;
% % %Shape: Rectangle [id:dp5408401972790353] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (126.95,95.93) -- (152.69,95.93) -- (152.69,123.42) -- (126.95,123.42) -- cycle ;
% % %Shape: Rectangle [id:dp09617849027584047] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (175.98,95.93) -- (201.73,95.93) -- (201.73,123.42) -- (175.98,123.42) -- cycle ;
% % %Shape: Rectangle [id:dp5343581467883038] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (292.76,95.93) -- (318.5,95.93) -- (318.5,123.42) -- (292.76,123.42) -- cycle ;
% % %Shape: Rectangle [id:dp9463661331926414] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (405.72,92.47) -- (429.95,92.47) -- (429.95,118.03) -- (405.72,118.03) -- cycle ;
% % %Shape: Rectangle [id:dp5495817686500137] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (363.26,44.47) -- (387.49,44.47) -- (387.49,70.03) -- (363.26,70.03) -- cycle ;
% % %Shape: Rectangle [id:dp724038687226743] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (446.27,44.47) -- (470.5,44.47) -- (470.5,70.03) -- (446.27,70.03) -- cycle ;
% % %Down Arrow [id:dp7880401552551355] 
% % \draw   (438.38,85.56) -- (439.94,86.86) -- (451.63,72.77) -- (454.74,75.36) -- (443.05,89.45) -- (444.61,90.74) -- (437.02,93.54) -- cycle ;
% % %Shape: Rectangle [id:dp15916921420340646] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (365.26,140.47) -- (389.49,140.47) -- (389.49,166.03) -- (365.26,166.03) -- cycle ;
% % %Shape: Rectangle [id:dp24045677945615296] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (448.27,140.47) -- (472.5,140.47) -- (472.5,166.03) -- (448.27,166.03) -- cycle ;
% % %Down Arrow [id:dp7330223135447826] 
% % \draw   (447.26,121.73) -- (445.73,123.05) -- (457.71,136.9) -- (454.64,139.55) -- (442.66,125.7) -- (441.13,127.03) -- (439.62,119.08) -- cycle ;
% % %Down Arrow [id:dp6842535363592126] 
% % \draw   (397.63,126.64) -- (396.08,125.33) -- (384.32,139.36) -- (381.21,136.76) -- (392.98,122.73) -- (391.42,121.43) -- (399.03,118.67) -- cycle ;
% % %Shape: Rectangle [id:dp8747976589531903] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (224.98,95.93) -- (250.73,95.93) -- (250.73,123.42) -- (224.98,123.42) -- cycle ;
% % %U Turn Arrow [id:dp8641820196640331] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (238.45,93.28) -- (238.45,86.3) .. controls (238.45,85.34) and (239.22,84.56) .. (240.19,84.56) -- (273.64,84.56) .. controls (274.6,84.56) and (275.38,85.34) .. (275.38,86.3) -- (275.38,87.46) -- (275.97,87.46) -- (274.07,91.53) -- (272.18,87.46) -- (272.77,87.46) -- (272.77,87.17) .. controls (272.77,87.17) and (272.77,87.17) .. (272.77,87.17) -- (241.06,87.17) .. controls (241.06,87.17) and (241.06,87.17) .. (241.06,87.17) -- (241.06,93.28) -- cycle ;
% % %U Turn Arrow [id:dp2678890809121517] 
% % \draw   (272.58,125.16) -- (272.58,133.81) .. controls (272.58,135.94) and (270.86,137.67) .. (268.73,137.67) -- (243.33,137.67) .. controls (241.2,137.67) and (239.47,135.94) .. (239.47,133.81) -- (239.47,131.24) -- (238.22,131.24) -- (241.35,127.66) -- (244.47,131.24) -- (243.22,131.24) -- (243.22,133.81) .. controls (243.22,133.87) and (243.27,133.92) .. (243.33,133.92) -- (268.73,133.92) .. controls (268.78,133.92) and (268.83,133.87) .. (268.83,133.81) -- (268.83,125.16) -- cycle ;

% % % Text Node
% % \draw (84.08,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{1}};
% % % Text Node
% % \draw (268.29,100.46) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% % % Text Node
% % \draw (131.56,172.84) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {incremental update};
% % % Text Node
% % \draw (373.03,175.45) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Meta-analysis};
% % % Text Node
% % \draw (149.4,63.25) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Round 1};
% % % Text Node
% % \draw (149.79,145.7) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] { Round 2};
% % % Text Node
% % \draw (133.52,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{2}};
% % % Text Node
% % \draw (182.56,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{3}};
% % % Text Node
% % \draw (299.33,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{k}};
% % % Text Node
% % \draw (411.41,96.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{1}};
% % % Text Node
% % \draw (410.04,143.3) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% % % Text Node
% % \draw (368.95,48.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{2}};
% % % Text Node
% % \draw (451.96,48.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{3}};
% % % Text Node
% % \draw (370.95,144.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{4}};
% % % Text Node
% % \draw (453.96,144.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{K}};
% % % Text Node
% % \draw (231.56,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{4}};


% % \end{tikzpicture}
% % \caption{ A diagram contrasting the incremental update algorithm with the classic meta-analysis algorithm. K local sites are shown. The dashed arrow indicate the steps that sequentially update average treatment effect estimates and propensity score model estimates. The solid-line arrows indicate the distributive nature of meta-analysis approach }
%     \label{figure:my_label}



%     \centering

%     \caption{Caption}
%     \label{fig:my_label}

% \end{figure}





==> ENAR_Mengtong__Copy_/propensity_score_estimates.tex <==

\begin{table}[]
\begin{tabular}{lrllrll}
\hline
                                                                     & \multicolumn{6}{c}{Propensity Score Estimates for Basal Insulin Treatment}                                                                          \\ \hline
                                                                     & \multicolumn{3}{l}{``Gold-standard'' from combined data}                         & \multicolumn{3}{l}{Collaborative inference method}                       \\
\multicolumn{1}{c}{}                                                 & Estimates & \multicolumn{1}{c}{Std.Errors} & \multicolumn{1}{l}{p-value} & Estimates & \multicolumn{1}{c}{Std.Errors} & \multicolumn{1}{c}{p-value} \\
Gender                                                               & 0.13      & 0.30                           & 0.72                        & 0.13      & 0.30                           & 0.67                        \\
Age                                                                  & -0.01     & 0.01                           & 0.39                        & -0.01     & 0.01                           & 0.46                        \\
\begin{tabular}[c]{@{}l@{}}Family diabetes\\ history\end{tabular}    & 0.72      & 0.44                           & 0.10                        & 0.72      & 0.44                           & 0.10                        \\
First transplant                                                     & 0.03      & 0.46                           & 0.97                        & 0.02      & 0.46                           & 0.95                        \\
\begin{tabular}[c]{@{}l@{}}Glomerular \\ disease\end{tabular}        & -0.33     & 0.32                           & 0.31                        & -0.33     & 0.32                           & 0.32                        \\
\begin{tabular}[c]{@{}l@{}}Polycystic kidney \\ disease\end{tabular} & -0.41     & 0.36                           & 0.24                        & -0.42     & 0.35                           & 0.25                        \\
Living Doner                                                         & 0.86      & 0.45                           & 0.05                        & 0.87      & 0.45                           & 0.05                        \\ \hline
\end{tabular}
\caption{Propensity score estimates from combined data via centralized analysis and collaborative inference method. We use 2R-GLO algorithm for estimating collaborative inference ``global" PS parameters. The resulting estimates are very close indicating that estimating propensity score using collaborative inference method is valid.}
\label{tab:ps-table}
\end{table}

==> ENAR_Mengtong__Copy_/simulation_infrequent.tex <==

\begin{table}[]
\begin{center}
    

\begin{tabular}{lccccc}
\hline
                                                               & \multicolumn{5}{c}{n=80,  K=5, $P(Y=1| k=5) = 0.05$}                                                                         \\ \hline
\multicolumn{1}{c}{\textit{Methods}}                           & \textit{Fails(\%)} & \textit{CP(\%)} & \textit{ABias$ 10^{-3}$} & \textit{ASE$\times 10^{-3}$} & \textit{ESE$\times10^{-3}$} \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{Oracle}} & 0.00               & 94.3            & 212                      & 258                          & 266                         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{3R-GLO}} & 0.00               & 94.4            & 210                      & 257                          & 264                         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{2R-GLO}} & 0.06               & 92.2            & 210                      & 241                          & 264                         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{1R-GLO}} & 0.07               & 91.7            & 225                      & 249                          & 301                         \\
\textit{Meta}                                                  & 61.41              & 91.3            & 233                      & 258                          & 291                         \\ \hline
                                                               & \multicolumn{5}{c}{n=80, K=5,  $P(Y=1| k=5) = 0.3$}                                                                          \\ \hline
\multicolumn{1}{c}{\textit{Methods}}                           & \textit{Fails(\%)} & \textit{CP(\%)} & \textit{ABias$ 10^{-3}$} & \textit{ASE$\times 10^{-3}$} & \textit{ESE$\times10^{-3}$} \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{Oracle}} & 0.00               & 94.5            & 211                      & 260                          & 266                         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{3R-GLO}} & 0.00               & 94.4            & 211                      & 259                          & 270                         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{2R-GLO}} & 0.08               & 94.5            & 211                      & 263                          & 270                         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{222222} \textit{1R-GLO}} & 0.08               & 94.0            & 225                      & 268                          & 343                         \\
\textit{Meta}                                                  & 1.36               & 91.5            & 230                      & 253                          & 289                         \\ \hline
\end{tabular}
\end{center}
\caption{Simulation results for both equal outcome prevalence across sites and unequal outcome prevalence across sites. 'Fails' stands the number of non-convergence for incremental methods and the traditional meta-analysis method over $25000$ replications. 'CP', 'Abias', 'ASE', 'ESE' stand for the coverage probability, the average absolute bias, the averaged estimated standard error of the estimates, and the empirical standard error respectively. $Pr(Y=1|k=5)$ is the pre-assigned proportion of events at the $5$th site. $Pr(Y=1|k=5) = 0.3$ mimics the setting where all sites have equal proportion of events, and $Pr(Y=1|k=5) = 0.3$ mimics the setting where the $5$th site has rarer proportion of events compared to the rest of the sites. 
% The percentage of calculation failures for Meta is 61.41\% in unbalanced case, and the percentages of calculation failures for incremental methods are significantly fewer than that of Meta estimator in both balanced and unbalanced cases. 
Both oracle estimation (i.e. the gold standard obtained by the centralized analysis) and the proposed incremental estimator 3R-GLO have Abias and CP very close to each other, either when the $5$th site has equal proportion or unequal proportion of events. This confirms the theoretical results given in Section ~\ref{sec:Asymptotics}. The Abias of 2R-GLO is the same as 3R-GLO. The CPs of 2R-GLO, 1R-GLO and 3R-GLO are close to Oracle as $Pr(Y=1|k=5)$ increases to the balanced event proportion $0.3$. In the Meta estimator (the inverse-variance weighted meta method), Abias, ASE and ESE are all larger than that in Oracle, 3R-GLO, 2R-GLO, and 1R-GLO. The coverage probability in the meta is consistently around $91.5\%$ not affected by $Pr(Y=1|k=5)$. }
\label{tab:simulation}
\end{table}
